Let Me Show You: Learning by Retrieving from Egocentric Video for Robotic Manipulation

Robots operating in complex and uncertain environments face considerable challenges. Advanced robotic systems often rely on extensive datasets to learn manipulation tasks. In contrast, when humans are faced with unfamiliar tasks, such as assembling a chair, a common approach is to learn by watching video demonstrations. In this paper, we propose a novel method for learning robot policies by Retrieving-from-Video (RfV), using analogies from human demonstrations to address manipulation tasks. Our system constructs a video bank comprising recordings of humans performing diverse daily tasks. To enrich the knowledge from these videos, we extract mid-level information, such as object affordance masks and hand motion trajectories, which serve as additional inputs to enhance the robot model's learning and generalization capabilities. We further feature a dual-component system: a video retriever that taps into an external video bank to fetch task-relevant video based on task specification, and a policy generator that integrates this retrieved knowledge into the learning cycle. This approach enables robots to craft adaptive responses to various scenarios and generalize to tasks beyond those in the training data. Through rigorous testing in multiple simulated and real-world settings, our system demonstrates a marked improvement in performance over conventional robotic systems, showcasing a significant breakthrough in the field of robotics.

==> task_description.tex <==
\begin{itemize}
    \item (Short horizon) \textbf{PlaceBread:} The robot is tasked with picking up a piece of bread from the desk and placing it on a plate. Both the bread and the plate are randomly placed during the evaluation.

    \item (Short horizon) \textbf{PlaceBall:} This task requires the robot to pick up a tennis ball and place it into a tennis ball box. The tennis ball is small, which makes it challenging for the robot to grasp. The box is exactly the size of the ball, demanding high precision for placement. Both objects are randomly placed during the evaluation.

    \item (Short horizon) \textbf{PlaceCan:} The robot must pick up a small and rigid can and place it into a cup holder. This task requires extreme precision due to the small size of the can. All objects are randomly placed during the evaluation.

    \item (Short horizon) \textbf{CloseLaptop:} The task involves closing a laptop, which is an articulated object. The laptop is randomly placed on the table during the evaluation. 

    \item (Short horizon) \textbf{SetCup:} The robot is tasked with setting a cup upright on the table. The cup is randomly placed on the table during the evaluation.

    \item (Short horizon) \textbf{InsertPlug:} The robot must insert a plug into a socket. The position of the socket is fixed, while the plug is randomly placed on the table during the evaluation. 
    
    \item (Long horizon) \textbf{CleanTable:} This multi-step task requires the robot to open a drawer, place a cube inside, and then close the drawer. Both the drawer and the cube are randomly placed on the table, adding complexity to the task.

    \item (Long horizon) \textbf{PackCube:} The robot must open the lid of a box, place a cube inside the box, and then close the lid. The box and the cube are randomly placed on the table during the evaluation.
\end{itemize}
